Dynamics of Evolving Social Groups

Exclusive social groups are ones in which the group members decide whether or not to admit a candidate to the group. Examples of exclusive social groups include academic departments and fraternal organizations. In the present paper we introduce an analytic framework for studying the dynamics of exclusive social groups. In our model, every group member is characterized by his opinion, which is represented as a point on the real line. The group evolves in discrete time steps through a voting process carried out by the group's members. Due to homophily, each member votes for the candidate who is more similar to him (i.e., closer to him on the line). An admission rule is then applied to determine which candidate, if any, is admitted. We consider several natural admission rules including majority and consensus. We ask: how do different admission rules affect the composition of the group in the long term? We study both growing groups (where new members join old ones) and fixed-size groups (where new members replace those who quit). Our analysis reveals intriguing phenomena and phase transitions, some of which are quite counterintuitive.

==> full/full-majority.tex <==
\begin{theorem} \label{thm-majority}
Consider a group $S$ of initial size $k_0$. For $k_{min}\geq \Theta((k_0)^2)$, with probability $(1-\sum_{k=k_{min}}^\infty e^{-\Theta(k^{1/5})})$: for any $\eps$ there exists $k_\eps > k_{min}$ such that for every $k'>k_{\eps}$ we have that $|m(S(k'))-\frac{1}{2}| < 3\eps$.
\end{theorem}

We begin by providing a few claims and lemmas that will be useful for proving the theorem.
The first lemma is the heart of the proof showing, roughly speaking, that if the median is at distance of $\dm$ to the left of $1/2$, then more members will be added to the group to the right of the median than to its left. Thus the median should move to the right. In the next claims we analyze by how much should the median move to the right. We note that for simplicity all claims and lemmas are stated and proven for the case in which the median is less than $1/2$. The proofs for the symmetric case in which the median is greater than $1/2$ are identical.

\begin{lemma} \label{lem:more-right}
Consider a group $S(k)$, such that $m(S(k))<\frac{1}{2}$. Let $\dm(k)=\frac{1}{2}-m(S(k))$. Assume that each of the intervals $[m(S(k))-\phi, m(S(k))]$ and $[m(S(k)), \frac{1}{2}-\frac{\dm(k)}{2}]$ includes at least $t$ members. Then, when adding $t$ more members to the group, with probability ($1-e^{-\frac{\dm(k)^4}{32} (\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi ) \cdot  t  }$) at least $t\cdot (\frac{1}{2} + \frac{\dm(k)^2}{4}-2\phi)$ newly added members will be added to the interval $[m(S(k)),1]$.
\end{lemma}
\begin{proof}
Note that since for the group $S(k)$ each of the intervals $[m(S(k))-\phi, m(S(k))]$ and $[m(S(k)), \frac{1}{2}-\frac{\dm(k)}{2}]$ contains at least $t$ members, for every step $k<k'<k+t$, we have that $m(S(k))-\phi \leq m(S(k')) \leq \frac{1}{2}-\frac{\dm(k)}{2}$. Consider a step $k'$ ($k < k' < k+t$) the probability of accepting a candidate above $m(S(k'))$ in this round is $\frac{1}{2} + 2\dm(k')^2$ by the following reasoning:
\begin{itemize}
\item With probability $4\dm(k')^2$ a candidate in the interval $[2m(S(k')),1]$ will join the group. The reason for this is that a candidate in this interval, which is the farthest from $m(S(k'))$, can only be accepted if the other candidate is in this interval as well. 
\item  By symmetry the probability of the candidate that joins to be in $[0,m(S(k'))]$ is the same as the probability to be in $[m(S(k')),2m(S(k'))]$. Hence the probability for the candidate to be in $[m(S(k')),2m(S(k'))]$ is $\frac{1-4\dm(k)^2}{2}$.
\end{itemize}
It is easy to see that the probability of adding a member above $m(S(k'))$ is decreasing as $m(S(k'))$ gets closer to $\frac{1}{2}$. As we assume that $m(S(k')) \leq \frac{1}{2}-\frac{\dm(k)}{2}$, the minimal probability for accepting above $m(S(k'))$ is $\frac{1}{2}+\frac{\dm(k)^2}{2}$. Also by the assumption that $m(S(k))-\phi \leq m(S(k'))$ we get that at least with this probability a member above $m(S(k))-\phi$ will join the group. As the probability of a member to join the interval $[m(S(k))-\phi, m(S(k))]$ is always at most $2\phi$, we get that the probability of a candidate to join above $m(S(k))$ is at least $\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi$. The proof is completed by the following Chernoff 
(c.f., e.g., \cite{alonProb}, appendix A). Denote by $R$ the number of steps in which a candidate above $m(S(k))$ was accepted:
\begin{align*}
Pr[R \leq (1- \frac{\dm(k)^2}{4})(\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi) \cdot t ] 
&\leq e^{-\frac{(\frac{\dm(k)^2}{4})^2 \cdot (\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi) \cdot t  }{2} } 
%\leq e^{-(\frac{\dm(k)^4}{64} +\frac{\dm(k)^2}{4} -2\frac{\phi}{2} ) \cdot  t  }
= e^{-\frac{\dm(k)^4}{32} (\frac{1}{2}+\frac{\dm^2}{2}-\phi ) \cdot  t  }
\end{align*}
Thus, with probability $(1-e^{-\frac{\dm(k)^4}{32} (\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi ) \cdot  t  })$, at least $(1- \frac{\dm(k)^2}{4})(\frac{1}{2}+\frac{\dm(k)^2}{2}-2\phi) \cdot t \geq (\frac{1}{2} + \frac{\dm(k)^2}{4}-2\phi) t$ members above $m(S(k))$ will be accepted. 
\end{proof}

We now prove bounds on the density of the group in every interval and every step. Let $\eps(k) = k^{-\frac{1}{10}}$ and $\is = (\frac{\eps(k)}{26})^4$. We begin by partitioning the $[0,1]$ interval into equal segments of length $\is /2$.

\begin{lemma} \label{lem:delta0_segments}
Consider $t$ time steps, then, the following holds with probability ($1-\frac{4}{\is}e^{- \frac{\is^2 t}{160}}$) for every segment $J$ in our $\is /2$-partition : 
\begin{enumerate}
\item The number of members accepted in these $t$ steps to $J$ is at most $\frac{3}{2} \cdot t \cdot \is $.
\item If $J$ is contained in $[0.1,0.9]$, then the number of members accepted in $t$ steps
to $J$ is at least $\frac{1}{40} \cdot t \cdot \is$.
%\item If $J$ is  in $[0,0.1]$ or $[0.1,0.9]$, then it includes at least a single member.
\end{enumerate}
\end{lemma}
\begin{proof}
We first compute the probability that a specific interval $J$ has the right number of candidates and then use a union bound to show that the lemma holds for all intervals simultaneously. Throughout this proof we denote the number of candidates in an interval $J$ by $X_J$.
\begin{enumerate}
\item \textbf{Upper bound -}Observe that with probability of at most $2\cdot \frac{\is}{2}$ at least one of the candidates is located in the interval $J$. This is clearly an upper bound on the probability of accepting a member in this interval and hence in expectation the number of group members in interval $J$ in the $t$ steps is at most $\is t$. By taking a Chernoff bound we get that the probability of accepting more than $\frac{3}{2} \is t$ group members in $J$ is at most:
\begin{align*}
Pr[X_J \geq (1 + 0.5)\is t  ] \leq e^{-\frac{ \frac{1}{4} \is t}{3}}
= e^{-\frac{ \is t}{12}}.
\end{align*}
\item \textbf{Lower bound $J \subset [0.1,0.9] $ -} A candidate $x$ in an interval $J$ in $[0.1,0.9]$ has a probability of at least $\frac{\is}{2} \cdot \frac{1}{10}$ of being selected. The reason being that if $m(S(k'))<1/2$, then a candidate $x$ in $J$ is closer to the median than any candidate in $[0.9,1]$. Similarly, if $m(S(k'))>1/2$, $x$ is preferred over any candidate in $[0,0.1]$. By taking Chernoff bounds we get that the probability of accepting less than $\frac{\is}{40} t$ group members in $J$ is at most:
\begin{align*}
Pr[X_J \leq (1 - 0.5) \frac{\is}{20} t  ] \leq e^{-\frac{ \frac{1}{4} \frac{\is}{20}t}{2}}
= e^{-\frac{ \is t}{160}}.
\end{align*}
%\item \textbf{Lower bound $J \subset [0,0.1]$ or $J \subset [0.9,1]$ -} For every segment $J$ of length $\frac{\is}{2}$ the probability that both candidates are in $J$ is $\frac{\is^2}{4}$. 
%Hence, with probability at least $\frac{\is^2}{4}$ a candidate in $J$ is chosen
%for the group. Thus in expectation there are at least $\mu_J=\frac{\is^2}{4} t$ group members in $J$.
%By taking Chernoff bounds we get that the probability of not accepting any member in $J$ is at most:
%\begin{align*}
%Pr[X_J \leq (1 - \frac{\mu_J-1}{\mu_j} ) \mu_J  ] \leq e^{-\frac{ (\frac{\mu_J-1}{\mu_j})^2 \mu_J}{2}} = 
%e^{- \frac{(\mu_J-1)^2}{2\mu_j}} \leq e^{- \frac{\mu_J}{3}} = e^{- \frac{\is^2 t}{12}}.
%\end{align*}
\end{enumerate}

Finally we take a union bound to show that all the segments have the right number of members with high probability:
\begin{align*}
\frac{2}{\is} (e^{-\frac{ \is t}{12}} + e^{-\frac{ \is t}{160}} ) 
\leq \frac{4}{\is}e^{- \frac{\is^2 t}{160}} 
\end{align*}
\end{proof}

Next, we use the bounds on the smaller consecutive intervals to show that any interval of length greater than $\is$ contains the ``right'' number of members:
\begin{claim} \label{clm-density-in-delta-intervals}
Let $k \geq \frac{k_0}{\is}$, for any interval $I$ of length 
$|I| \geq \is$ the following holds with probability $(1-\frac{4}{\is}e^{- \frac{\is^2 k}{320}})$ :
\begin{enumerate}
\item The number of members in $I$ is at most $7 |I| \cdot k$.
\item For any interval contained in $[0.1,0.9]$ the number of members
in $I$ is at least $|I| \cdot k/120$.
%\item Every interval contained in $[0,0.1]$ or $[0.1,0.9]$ includes at least a single member.
\end{enumerate}
\end{claim}
\begin{proof}
In Lemma \ref{lem:delta0_segments} we partitioned the interval $[0,1]$ to disjoint segments of length $\frac{\is} {2}$ and proven that each one has the ``right'' number of group members. To show that similar density bounds holds for \emph{any} interval of length at least $\is$, we observe that any interval of size $|I|$ is contained in an interval $I^l$ of length at most $\is + |I|$ consisting of consecutive segments of our $\is/2$-partition and contains an interval $I^s$ of length at least $\max \{|I|-\is,\frac{\is}{2}\} \geq |I| /3$ of consecutive segments of the $\is/2$-partition. Thus, we can apply Lemma \ref{lem:delta0_segments}. For the upper bound this implies that each segment of length $\frac{\is}{2} $ contains at most $3 \cdot \frac{\is}{2} (k-k_0)$ candidates. Thus the interval $I^l$ includes at most $(3 \is + 3|I|) (k-k_0) < 6 |I| |k-k_0|$ members who joined the group in the admission process. Now, by observing that in the worst case all the $k_0$ initial members were located in this interval we have that the number of members in this interval is at most $6 |I| |k-k_0|+k_0$ by the assumption that $k \geq \frac{k_0}{\is}$ we have that $6 |I| |k-k_0|+k_0 \leq 7|I| \cdot k$. As for the lower bound, by applying Lemma \ref{lem:delta0_segments} we have that the interval $I^s$ (and hence the interval $I$) contains at least $\frac{|I|}{60} (k-k_0)$ members which is more than $\frac{|I|}{120} k$ by the assumption that $k \geq 2k_0$.

\end{proof}

Now we would like to use the density bound we computed in the previous claim to bound by which distance a median that was initially left of $1/2$ should move to the right. However, since the density bounds only hold when the median is in the interval $[0.1,0.9]$ we begin by considering separately the case in which the median is less than $0.2$. 
\begin{claim} \label{clm-edge-interval}
If $m(S(k))< 0.2$, then with probability $(1-2e^{-\frac{k}{1000}})$ we have that $m(S(6k)) \in [0.2,0.8]$.
\end{claim}
\begin{proof}
We first observe that the probability of accepting a candidate in $[0.2,1]$ is at least $0.64$ since with this probability both candidates will be in this interval and we will have to accept one of them. Consider increasing the size of the group $S(k)$ by $5k$ more members. In expectation at least $5 \cdot k \cdot 0.64 = 3.2 k$ of those members should be in the interval $[0.2,1]$. Let $X$ denote the number of members accepted in the interval $[0.2,1]$, by taking a Chernoff bound we get that with probability $(1-e^{-\frac{k}{1000}})$ $X \geq (1-0.03) \cdot 3.2 k \geq 3.1 k$:
\begin{align*}
Pr[X \leq (1-0.03) \cdot 3.2 k] \leq e^{-\frac{0.03^2 \cdot 3.2 k }{2}} \leq e^{-\frac{k}{1000}}
\end{align*}
Thus, with this probability the median of the group $S(6k)$ has to be above $0.2$. For the same reason after these $5k$ steps the median should be below $0.8$ and hence it has to be in the interval $[0.2,0.8]$.
\end{proof}

Next, we use the density bounds computed in the previous claim, to bound by how much a median in the interval $[0.2,0.5) $ should move to the right: 
\begin{claim}\label{clm:small-step}
If $m(S(k))>0.2$ and $m(S(k)) = \frac{1}{2} - \dm(k)$ and $\dm(k) > \eps(k)$, then with probability $1-2\frac{4}{\is}e^{- \frac{\is^2 k}{320}}-e^{-k \cdot(\frac{\dm(k)}{10})^4 }$, we have that $\frac{1}{2} -  m(S(k+\step \cdot k)) \leq \dm(k) - (\frac{\dm(k)}{26})^4$.
\end{claim}
\begin{proof}
We first observe that by the assumption that $\dm(k) > \eps(k)$ we have that $\frac{\dm(k)^2}{16} > \is $ (recall that $\is = (\frac{\eps(k)}{26})^4 $). Also, by the assumption that $m(S(k))>0.2$ we have that $m(S(k))-\frac{\dm(k)^2}{16} > 0.1$ and hence we can apply Claim \ref{clm-density-in-delta-intervals} for the group $S(k)$, and get that each of the intervals $[m(S(k))-\frac{\dm(k)^2}{16}, m(S(k))]$ and $[m(S(k)), m(S(k))+\frac{\dm(k)^2}{16}]$ contain at least $\step \cdot k$ members. Hence with probability $1-\frac{6}{\is}e^{- \frac{\is^2 k}{320}} $, we have that in the next $\step \cdot k$ the median is always in the interval $[m(S(k))-\frac{\dm(k)^2}{16}, m(S(k)) + \frac{\dm(k)^2}{16}]$. Thus, we can apply Lemma \ref{lem:more-right} and get that with probability:
\begin{align*}
 (1-e^{-\frac{\dm(k)^4}{32} (\frac{1}{2}+\frac{\dm(k)^2}{2}-\frac{\dm(k)^2}{8} ) \cdot  \step \cdot k  }) \geq 
(1-e^{-k \cdot(\frac{\dm(k)}{10})^6}),
\end{align*} 
$\step \cdot k \cdot (\frac{1}{2} + \frac{\dm^2}{4}-2\cdot \frac{\dm^2}{16})$ new members will join to the right of $m(S(k))$. This implies that the median will move to the right by at least $\frac{\dm^2}{16} \cdot \frac{\dm^2}{1920} \cdot k = (\frac{\dm^4}{30720}) \cdot k$ members. 

Next, we observe that with probability of at least $1-\frac{4}{\is}e^{- \frac{\is^2 k}{320}} $ the bounds from Claim \ref{clm-density-in-delta-intervals} also hold for the group $S(k + \step \cdot k)$ (this is because this probability increases as $k$ is increasing.). Thus every interval of size $|I| \geq \delta(k) > \delta(k + \step \cdot k)$ contains at most $7 \cdot |I| \cdot (k + \step \cdot k) < 14 \cdot |I| \cdot k $ points. In particular this implies that since $(\frac{\dm}{26})^4 > \delta(k)$, then the interval $[m(S(k)), m(S(k)+(\frac{\dm(k)}{26})^4]$ contains less than $\frac{\dm(k)^4}{30720} \cdot k$ members. Thus, after $\step \cdot k$ steps the median should move a distance of at least $(\frac{\dm(k)}{26})^4$ to the right -- $\frac{1}{2} - m(S(k + \step \cdot k)) \leq \dm(k) - (\frac{\dm(k)}{26})^4$.

The proof is completed by taking a union bound on the three bad events and hence we have that with probability $1-2\frac{6}{\is}e^{- \frac{\is^2 k}{320}}-e^{-k \cdot(\frac{\dm(k)}{10})^6 }$ the claim holds.
\end{proof}

The last case we need to handle is the one in which $\dm(k) < \eps(k)$.
\begin{claim} \label{clm-close}
If $\dm(k) < \eps(k)$, then with probability $(1-\frac{4}{\is}e^{- \frac{\is^2 k}{320}})$ for any $k< k' < k+\frac{\eps(k)}{120} \cdot k$, $|\frac{1}{2} - m(S(k'))| < 2 \eps(k) <4\eps(k')$.
\end{claim}
\begin{proof}
Observe that since by definition $\eps(k) > \is$ then for the group $S(k)$, with probability $(1-\frac{4}{\is}e^{- \frac{\is^2 k}{320}})$ each of the intervals $[m(S(k))-\eps(k),m(S(k))]$ and $[m(s(k)),m(S(k))+\eps(k)]$ contains at least $\frac{\eps(k)}{120} \cdot k$ members. Hence, in $\frac{\eps(k)}{120} \cdot k$ steps the median can move a distance of at most $\eps(k)$. The proof is completed by recalling that $\eps(k+ \frac{\eps(k)}{120} \cdot k) > \eps(2k) > \frac {\eps(k)}{2}$.
\end{proof}
 
%\begin{theorem}
%For every $\eps$, there exists $k_\eps$ such that for any $k' \geq k_\eps$ with probability $()$ we have that $|m(S(k'))-\frac{1}{2}| < 3\eps$.
%\end{theorem}

We now state again the theorem we prove:
\begin{theorem*}
Consider a group $S$ of initial size $k_0$. For $k_{min}\geq 26^8 \cdot (k_0)^2$, with probability of at least $(1-20^5 \cdot \sum_{k=k_{min}}^\infty e^{-\frac{k^{\frac{1}{5}}}{20^7}})$: for any $\eps$ there exists $k_\eps > k_{min}$ such that for every $k'>k_{\eps}$ we have that $|m(S(k'))-\frac{1}{2}| < 3\eps$.
\end{theorem*}

\begin{proof}
Recall that $\eps(k) = k^{-\frac{1}{10}}$ and $\is = (\frac{\eps(k)}{26})^4$. If $m(S(k_{min}))<0.2$ or $m(S(k_{min}))>0.8$, then we begin by applying Claim \ref{clm-edge-interval} that shows that with probability of at least $1-e^{-\frac{k_{min}}{1000}}$, $m(S(6k_{min})) \in [0.2,0.8]$. Once the median is in this middle interval We prove the theorem by applying 
Claim \ref{clm:small-step} and Claim \ref{clm-close} infinitely many times (the two claims also imply that the median can never leave the interval $[0.2,0.8]$.):
\begin{itemize}
\item If $|m(S(k))-\frac{1}{2}|>\eps(k)$, let $\dm(k) = |\frac{1}{2} - m(S(k))|$.
 In this case, we can use Claim \ref{clm:small-step} to show that
 $|\frac{1}{2} -  m(S(k+\frac{\dm(k)^2}{1920} \cdot k))| \leq \dm(k) - (\frac{\dm(k)}{26})^4$.
\item Else, $|m(S(k))-\frac{1}{2}|<\eps(k)$ we can use Claim \ref{clm-close} to show that for any $k\leq k' \leq (1+\eps(k)) \cdot k$, $|m(S(k'))-\frac{1}{2}|<2\eps(k)$.
\end{itemize}
This implies that for any $\eps$, there exists $k_\eps$ such that $\eps(k_{\eps}) < \eps$ and $|m(S(k_\eps))-\frac{1}{2}|<\eps$. The reason is that as long as the median has not reached a distance of at least $\eps$ from $1/2$ each time we apply Claim \ref{clm:small-step} the distance will be reduced by at least $(\frac{\eps}{26})^4$. Moreover, since $\eps(k)$ is constantly decreasing we will apply Claim \ref{clm:small-step} sufficiently many times for the distance to be reduced. 

Once the group reached size $ k_\eps$ such that $|m(S(k_\eps))-\frac{1}{2}|<\eps$ and $\eps(k_{\eps}) < \eps$, we can continue applying the two claims for any $k\geq k_\eps$ and get that the median never moves more than a distance of $3 \eps$ from $\frac{1}{2}$:
\begin{itemize}
\item If $|m(S(k))-\frac{1}{2}|<\eps(k)$ we can use Claim \ref{clm-close} to show that for any $k\leq k' \leq (1+\eps(k)) \cdot k$, $|m(S(k'))-\frac{1}{2}|<2\eps(k) <2\eps$.
\item Else, $\eps(k) < |m(S(k))-\frac{1}{2}| < 2\eps(k)$. Let $\dm(k) = |\frac{1}{2} - m(S(k))|$.
 In this case, we can use Claim \ref{clm:small-step} to show that for any round $k'$ in the next $\frac{\dm(k)^2}{1920} \cdot k$ rounds, $|m(S(k'))-\frac{1}{2}| < 3 \eps (k) < 3\eps$ and $|m(S(k+\frac{\dm(k)^2}{1920} \cdot k))-\frac{1}{2}| <  |m(S(k))-\frac{1}{2}|$.
\end{itemize}
To prove that we can indeed use each of these claims infinity many times, we take a union bound over all the bad events that can happen during these applications. In particular, the first bad event is that for some $k'$ the density bounds for Claim \ref{clm-density-in-delta-intervals} do not hold. This happens with probability of at most:
\begin{align*}
\sum_{k=k_{min}}^\infty \frac{4}{\is}e^{- \frac{\is^2 k}{160}}  &= \sum_{k=k_{min}}^\infty \frac{4}{(\frac{k^{-\frac{1}{10}}}{26})^4}e^{- \frac{((\frac{k^{-\frac{1}{10}}}{26})^4)^2 k}{160}} = 
\sum_{k=k_{min}}^\infty 4 \cdot 26^4 \cdot k^{\frac{2}{5}} \cdot e^{-\frac{k^{\frac{1}{5}}}{160 \cdot 26^4}} \\ 
&=\sum_{k=k_{min}}^\infty 4 \cdot 26^4 \cdot e^{\ln(k^{\frac{2}{5}})} \cdot e^{-\frac{k^{\frac{1}{5}}}{160 \cdot 26^4}} \\ 
&=  4 \cdot 26^4 \cdot \sum_{k=k_{min}}^\infty e^{2\ln(k^{\frac{1}{5}})-\frac{k^{\frac{1}{5}}}{160 \cdot 26^4}} \\
&\leq (19.5)^5 \cdot \sum_{k=k_{min}}^\infty e^{-\frac{k^{\frac{1}{5}}}{20^7}}
\end{align*}

The second bad event is that the number of members we add on the side which is farthest from the median is not the one specified by Lemma \ref{lem:more-right} (which is on the lemmas we require for the correctness of Claim \ref{clm-close}). Again, by taking a union bound one of these bad event will happen with probability of at most:
 \begin{align*}
\sum_{k=k_{min}}^{\infty} e^{-k \cdot(\frac{\dm(k)}{10})^6 } &\leq
\sum_{k=k_{min}}^{\infty} e^{-k \cdot(\frac{\eps(k)}{10})^6 } =
\sum_{k=k_{min}}^{\infty} e^{-k \cdot(\frac{k^{-\frac{1}{10}}}{10})^6 } 
= \sum_{k=k_{min}}^{\infty} e^{- \frac{k^{\frac{4}{10} }}{10^6}}
\end{align*}

Where in the first transition we use the fact that $\dm(k) \geq \eps(k)$.
\end{proof}

==> full/full-non-extreme-sketch.tex <==
In the following subsections we first show that the $p$-quantile will get to a location greater than $1/2$ and stay there. Next, we show that given that the $p$-quantile is above $1/2$ it will converge to $\tau_p$.
\subsubsection{The $p$-quantile converges to a value greater than $1/2$}

%\begin{theorem} \label{thm-greater-than-half}
%Let $k_0$ be the initial size of the group. For $k_{min} > k_0$, with probability $1-  \sum_{k=k_{min}}^\infty e^{-\theta(k)}$, there exists $k_{1/2} >  k_{min}$ such that for every $k\geq k_{1/2}$, $q_p(S(k))>1/2$.
%\end{theorem}
Pick $\eps = \frac{p-1/2}{4}$, we show that:
\begin{theorem} \label{thm-greater-than-half}
Let $k_0$ be the initial size of the group. For $k_{min} > k_0$, with probability $1-\sum_{i=1}^{\infty} e^{-\Theta(\eps^3 (1+\eps)^{i-1} k_{min})}$, there exists $k_{1/2} > k_{min}$ such that $q_{p-\eps}(S(k_{1/2}))>1/2$.
\end{theorem}
\begin{proof}
The proof follows a very similar structure to the proof of Theorem \ref{thm:conv:extreme}. 
Pick $\eps = \frac{p-1/2}{4}$. We begin by showing that as we increase the group by $\eps k$ members at most $(p-2\eps) \cdot \eps k$ members will join the interval $[0, q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$.

\begin{claim} \label{clm:half-eps-k}
For a group $S(k)$ such that $q_{p-\eps}(S(k))<1/2$, consider adding $\eps k$ members to the group $S(k)$, with probability $(1-e^{-\Theta(\eps^3k)})$. The number of members that joined the interval $[0, q_{p-\eps}(S(k))+ \eps \cdot q_{p-\eps}(S(k))^2]$ in the $\eps k$ steps at most $(p-2\eps) \cdot \eps k$.
\end{claim}
\begin{proof}
Note that by definition we have that for every step $k'$ of the $\eps k$ steps, $q_{p}(S(k')) \geq q_{p-\eps}(S(k))$. We claim that this implies that the probability that the next accepted candidate is below $q_{p-\eps}(S(k)) + \eps \cdot q_{p-\eps}(S(k))^2$ is at most $p-3\eps$. To see why this is the case we first observe that with probability $ q_{p-\eps}(S(k))^2$ both candidates are below $q_{p-\eps}(S(k))$ and hence a candidate below $q_{p-\eps}(S(k))$ is accepted. Also note that with probability at most $2 \eps \cdot q_{p-\eps}(S(k))^2$ a member in the interval $[q_{p-\eps}(S(k)), q_{p-\eps}(S(k))+ \eps \cdot q_{p-\eps}(S(k))^2]$ joins the group, as this is an upper bound on the probability that a candidate in this interval shows up. Finally, as we only take into account steps in which a candidate was chosen we should divide the probabilities above by the probability of accepting a member. It it easy to see that the probability of accepting a member is minimized when $q_p(S(k')) = q_{p-\eps}(S(k))$ and hence the probability that the next accepted candidate is in the interval $[0, q_{p-\eps}(S(k))+ \eps \cdot q_{p-\eps}(S(k))^2]$ is at most 
\begin{align*}
\dfrac{q_{p-\eps}(S(k))^2 + 2 \eps \cdot q_{p-\eps}(S(k))^2}{2q_{p-\eps}(S(k))^2} = \dfrac{1}{2}+\eps = p-3\eps.
\end{align*}
By taking a Chernoff bound we get that with high probability the number of members accepted in the $\eps k$ steps in the interval $[0, q_{p-\eps}(S(k))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$ is at most $(p-2\eps) \cdot \eps k$. Denote by $X$ the number of candidates accepted in the interval $[0, q_{p-\eps}(S(k))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$, then
\begin{align*}
Pr[X\geq (1+\eps) \cdot (p-3\eps) \cdot \eps k] \leq e^{-\frac{\eps^2 (p-3\eps) \cdot \eps k}{3}} \leq e^{-\Theta(\eps^3k)}
\end{align*}
\end{proof}

Let $k_1=k_{min}$ and for any $i>1$ let $k_{i+1} = \eps k_i$. Also let $j=\lceil \log_{1+\eps} \frac{1}{\eps} \rceil$. We show that with high probability: $q_{p-\eps}(S(k_{i+j})) > q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2$.

\begin{claim} \label{clm-half-decreasing}
For $i>1$, with probability $(1-\sum_{l=1}^{j-1} e^{-\Theta(\eps^3 (1+\eps)^lk_i)})$, either there exists $k_i<k'<k_{i+j}$ such that $q_{p-\eps}(S(k))>1/2$ or $q_{p-\eps}(S(k_{i+j})) > q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2$.
\end{claim}
\begin{proof}
To prove the claim we apply Claim \ref{clm:half-eps-k} $j$ times. First we observe that with high probability for every $i$, $q_{p-\eps}(S(k_{i+1})) \geq q_{p-\eps}(S(k_i))$. The reason for this is that by Claim \ref{clm:extreme-eps-k} we have that the number of members that joined in the $\eps k_i$ steps between $k_i$ and $k_{i+1}$ in the interval $[0, q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$ is at most $(p-2\eps) \cdot \eps k$. Since the interval $[0, q_{p-\eps}(S(k_i))]$ is included in this interval we have that at most $(p-2\eps) \cdot \eps k$ members were admitted to it. Hence, $q_{p-\eps}(S(k_{i+1})) \geq q_{p-\eps}(S(k_i))$.

Next, we consider all the members in the $k_{i+j}-k_i$ steps. The fact that $q_{p-\eps}(S(k_{i+1})) \geq q_{p-\eps}(S(k_i))$ implies that in the $k_{i+j}-k_i$ the number of candidates admitted to the interval $[0, q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$ is at most $(p-2\eps)(k_{i+j}-k_i)$. We observe that in the worst case for the group $S(k_i)$ the interval $[0, q_{p-\eps}(S(k_i))+ \eps \cdot q_{p-\eps}(S(k_i))^2]$ contained $k_i$ points. Thus, to prove the claim, we should show that $(p-2\eps)(k_{i+j}-k_i)+k_i < (p-\eps)k_{i+j}$. Observe that 
\begin{align*}
(p-2\eps)\cdot(k_{i+j}-k_i) + k_i &= (p-\eps)k_{i+j} -\eps k_{i+j} + (1-p+2\eps)k_i  \\
&< (p-\eps)k_{i+j} - k_{i} + (1-p+2\eps)k_i \\
&< (p-\eps)k_{i+j}.
\end{align*}
For the second transition we used the fact that $k_{i+j} = (1+\eps)^{\lceil \log_{1+\eps} \frac{1}{\eps} \rceil} k_i > \frac{1}{\eps} k_i$.

Thus by taking a union bound over the bad events we get that the claim holds with probability
at least 
\begin{align*}
1-\sum_{l=i}^{i+j-1} e^{-\Theta(\eps^3 k_l)} = 1-\sum_{l=1}^{j-1} e^{-\Theta(\eps^3 (1+\eps)^lk_i)}
\end{align*}
\end{proof}
The proof of the theorem is completed by observing that we can apply Claim \ref{clm-half-decreasing} till we reach $k_{1/2}$ such that $q_{p-\eps}(k_{1/2})>1/2$. By taking a union bound over the bad events in the application of Claim \ref{clm-half-decreasing} we have that such $k_{1/2}$ exists with probability of at least:
\begin{align*}
1-\sum_{i=1}^{\infty} e^{-\Theta(\eps^3 k_i)} = 1-\sum_{i=1}^{\infty} e^{-\Theta(\eps^3 (1+\eps)^{i-1} k_1)}
\end{align*}
\end{proof}

Before moving to showing that the $p$-quantile Converges to $\tau_p$. We provide a Claim that will be useful to show that once the $(p-\eps)$-quantile is greater than half then with high probability essentially it will stay over $1/2$:
\begin{claim} \label{clm:non-stays}
If $q_{p-\eps}(S(k)) > 1/2$, then with probability $(1-e^{-\theta(k)})$, $q_{p-\eps}(S((1+\eps)k)) > 1/2$
\end{claim}
\begin{proof}
Observe that since $q_{p} (S(k')) >1/2$ for all $k'$ of the $\eps k$ steps, the expected number of members accepted below $1/2$ in these $\eps k$ steps is at most $\frac{\eps k}{2}$. By taking a Chernoff bound, we have that with probability $1-e^{-\frac{\eps^3 k}{6}}$ the number of candidates accepted in $[0,1/2]$ is at most $(1/2+\eps)\eps k$:
\begin{align*}
Pr[X\geq (1+\eps) \cdot \frac{1}{2} \eps k] \leq e^{-\frac{\eps^2 \frac{1}{2} \eps k}{3}} = e^{-\frac{\eps^3 k}{6}}
\end{align*}
The proof is completed by observing that $(1/2+\eps)<p-\eps = 1/2 + 3\eps$.
\end{proof}



\subsubsection{The $p$-quantile Converges to $\tau_p$}
We first compute the value of $\tau_p$. Recall that in the beginning of
the section we argued that when the $p$-quantile is above $1/2$ the probability of accepting a candidate left of $q_p(S(k))$ is $f(q_p(S(k)))=\frac{q_p(S(k))^2}{1-2(1-q_p(S(k)))^2}$. Given this, the value of $\tau_p$ can be computed as follows:
\begin{claim}
The fixed point for the location of the $p$-quantile is:$\tau_p = \frac{2p + \sqrt{2p^2-p}}{1+2p}$.
\end{claim}
\begin{proof}
As previously discussed since $\tau_p$ is a ``fixed point'' $(f(\tau_p)=p)$ then:
\begin{align*}
\frac{\tau_p^2}{1-2(1-\tau_p)^2} = p &\implies \tau_p^2 = p - 2p\tau_p^2 + 4p\tau_p -2p \\ &\implies (1+2p)\tau_p^2-4p\tau_p +p = 0.
\end{align*}
The solutions for this equation are
\begin{align*}
\tau_p = \frac{4p \pm \sqrt{16p^2 - 4p(1+2p)}}{2(1+2p)} = \frac{2p \pm \sqrt{2p^2-p}}{1+2p}.
\end{align*}
Recall that $f(q)$ is only defined for $q > 1/2$, thus we are only interested in points located above $1/2$. The only such point is $\tau_p = \frac{2p + \sqrt{2p^2-p}}{1+2p}$.
\end{proof}

The theorem we wish th prove is the following:
\begin{theorem*}
Consider a group $S$ of initial size $k_0$. For $k_{min}>k_0$, with high probability: for any $\dm$ there exists $k_\dm > k_{min}$ such that for every $k'>k_{\dm}$ we have that $|q_p(S(k))-\tau_p| < 2\dm$.
\end{theorem*}
The proof is very much similar to the proof of Theorem \ref{thm-majority} showing that the median converges to $1/2$, hence we only provide a sketch of it. First, in Claim \ref{clm:prob:comp}, which is provided below, we show that the probability accepting a candidate left of $q_p(S(k))>1/2$ for $q_p(S(k))=\tau_p-\dm(k)$ is less than $p-\varphi_1 \cdot \dm(k)$ for some constant $\varphi_1$. A similar claim shows that for $q_p(S(k))=\tau_p+\dm(k)$ this probability is at least $p+\varphi_2 \cdot \dm(k)$. Hence, roughly speaking, in both cases the $p$-quantile has to move closer to $\tau_p$. 

Next, we show that each interval $I\in [0.5,1]$ of length $\delta(k) = k^{-1/10}$ contains with high probability at least $c_1 \cdot (\delta(k) \cdot k)$ members and at most $c_2 \cdot (\delta(k) \cdot k)$. Therefore, we can increase the group by $k_{inc} = c_1 \cdot \delta(k) \cdot k $ members and have for any step $k<k'<k+k_{inc}$: $q_p(S(k))-\delta(k) <q_p(S(k')) < q_p(S(k))+\delta(k)$. 

From this point onwards to simplify the presentation we assume that $q_p(S(k))<\tau_p$; the proof for the case $q_p(S(k))>\tau_p$ is very similar. Observe that for $k'$ such that $q_p(S(k))-\delta(k) <q_p(S(k'))$ the probability of the next accepted candidate to be in the interval $[0,q_p(S(k))]$ is at most $p-\varphi_1 \cdot \dm(k) + 4\delta(k)$. The reason for this is that the probability of the next accepted candidate to be in the interval $[0,q_p(S(k))-\delta(k)]$ is less than $p-\varphi_1 \cdot \dm(k)$ and the probability of the next accepted candidate to lie in the interval $[q_p(S(k))-\delta(k),q_p(S(k))]$ is at most $4\delta(k)$, as the probability of a candidate showing up in this interval is at most $2\delta(k)$ and the probability of accepting any candidate is at least $1/2$. Hence, if $\dm(k) > 8\delta(k)$ then, the probability of the next accepted candidate to be in the interval $[0,q_p(S(k))]$ is at most $p-(\varphi_1/2)\dm(k)$. We can now take a Chernoff bound and get that with high probability in the $k_{inc}$ steps the $p$-quantile has moved right by at least $(\varphi_1/8) \cdot \dm(k) \cdot k_{inc} = (\varphi_1/8)\cdot \dm(k) \cdot c_1 \cdot \delta(k) \cdot k$ points.

Finally by the fact the each interval of length $\delta(k)$ contains at most $c_2 \cdot \delta(k) \cdot k$ points, we have that if $\dm(k)$ is sufficiently larger than $\delta(k)$
then $q_p(S(k))+c_3 \cdot \dm(k) \leq q_p(S(k+k_{inc})) < \tau_p$, for some constant $c_3$. By iterating over the previous arguments we get that indeed as the group grows the $p$-quantile gets closer to $\tau_p$.


\begin{claim} \label{clm:prob:comp}
There exist two positive functions $\varphi_1(p), \varphi_2(p)$, such that for $1/2<q_p(S(k))<\tau_p$, $f(\tau_p-\dm(k)) \leq p-\varphi_1(p) \cdot \dm(k)$ and for $q_p(S(k))>\tau_p$, $f(\tau_p+\dm(k)) \geq p+\varphi_2(p) \cdot \dm(k)$.
\end{claim}
\begin{proof}
As the size of the group does not play a role in this proof we define $\dm=\dm(k)$.
\begin{align*}
f(\tau_p-\dm) = \frac{(\tau_p-\dm)^2}{1-2(1-(\tau_p-\dm))^2} = \frac{\tau_p^2 -2\dm \tau_p + \dm^2}{1-2(1-\tau_p+\dm)^2} = \frac{ p \cdot (1-2(1-\tau_p)^2) -2\dm \tau_p + \dm^2}{1-2(1-\tau_p)^2 - 4\dm(1-\tau_p) -2\dm^2}.
\end{align*}
The last transition is by the definition of $\tau_p$ as a fixed point. We can further simplify this expression as follows:
\begin{align*}
= p+ \frac{ p\cdot(4\dm(1-\tau_p) -2\dm^2) -2\dm \tau_p + \dm^2}{1-2(1-(\tau_p-\dm))^2}
\leq p+   \dm(4p-2(1+2p)\tau_p) +\dm^2(1+2p).
\end{align*}
Note that we only care about cases that the numerator is negative, hence to get an upper bound we can use the assumption that the denominator is at most $1$. We now plug the value of $\tau_p$ and get:
\begin{align*}
= p+   \dm(4p-2(1+2p) \cdot \frac{2p + \sqrt{2p^2-p}}{1+2p}) +\dm^2(1+2p)
&= p+   \dm(4p-2 \cdot(2p + \sqrt{2p^2-p}) +\dm^2(1+2p)\\
&= p -2\dm \sqrt{2p^2-p} +\dm^2(1+2p).
\end{align*} 
Finally, we show that there exists a function $\varphi_1(p)>0$ such that for any $\dm < \tau_p-1/2 $ , $f(\tau_p-\dm) < p -\varphi_1(p) \cdot \dm$:
\begin{align*}
p-2\dm \sqrt{2p^2-p} +\dm^2(1+2p) < p-\varphi_1(p) \cdot \dm \implies \dm(\dm(1+2p)-2\sqrt{2p^2-p} +\varphi_1(p) ) <0
\end{align*}
The inequality holds for $\dm \in [0,\frac{2\sqrt{2p^2-p} -\varphi_1(p)}{1+2p}]$. Since, we want this to hold for any $\dm \in [0,\tau_p-1/2]$ we require that:
\begin{align*}
\frac{2\sqrt{2p^2-p} -\varphi_1(p)}{1+2p} > \frac{2p + \sqrt{2p^2-p}}{1+2p} - 1/2 \implies \varphi_1(p) <  \sqrt{2p^2-p} +1/2-p. 
\end{align*}
The proof is completed by observing that indeed for any $p>1/2$, $\sqrt{2p^2-p} +1/2-p>0$ and hence there exists $\varphi_1(p)$ as required.

A very similar computation shows that when $q_p(S(k))>\tau_p$, there exists a function $\varphi_2(p)$ such that $f(\tau_p+\dm(k)) \geq p+\varphi_2(p) \cdot \dm(k)$.
\end{proof}

==> full/full-non-extreme.tex <==
\begin{proof}
We begin by observing that for $q>1/2$ the admission rule is smooth. First, recall that for $q\geq 1/2$ we have that $f(q)=\frac{q^2}{1-2(1-q)^2}$. Note that due to the normalization it is indeed the case that each step a candidate is accepted to the group. Also, it is easy to verify that this is function is increasing and continuous for $q\in(1/2,1]$. Next, observe that for $q\in(1/2,1]$ the probability of accepting a candidate in every interval $\delta$ is at most $\frac{2\delta}{1-2(1-q)^2} \leq 4\delta$ and at least $\delta^2$. For the lower bound observe that the interval with the minimal acceptance probability is the last interval $[1-\delta,1]$. Now, by the geometric representation depicted in Figure \ref{fig-delta} a candidate in $[1-\delta,1]$ will be accepted if the point defined by the two candidates is in one of the striped triangles in the figure. Hence the total probability of accepting a candidate in $[1-\delta,1]$ is at least $\delta^2$. 

Now, by Theorem \ref{thm-general-converge} we have that the $p$-quantile of a smooth admission rule converge to $\tau_p=\frac{2p + \sqrt{2p^2-p}}{1+2p}$ with probability $1-o(1)$. In Theorem \ref{thm-veto-smooth} below we show that with high probability there exists some value of $k$ starting which the admission rule is always smooth. Thus, we have that with high probability the $p$-quantile of the group converges to $\tau_p$.
\end{proof}



%\begin{claim}
%The admission rule for $q>1/2$: $f(q)=\frac{q^2}{1-2(1-q)^2}$ is smooth.
%\end{claim}
%\begin{proof}
%First observe that due to the normalization it is indeed the case that each step a candidate is accepted to the group. Also, it is easy to verify that this is function is increasing and continuous for $q\in(1/2,1]$. Also, observe that for $q\in(1/2,1]$ the probability of accepting a candidate in every interval $\delta$ is at most $\frac{2\delta}{1-2(1-q)^2} \leq 4\delta$ and at least $\delta^2$. For the lower bound observe that the interval with the minimal acceptance probability is the last interval $[1-\delta,1]$. Now, by the geometric representation depicted in Figure \ref{fig-delta} a candidate in $[1-\delta,1]$ will be accepted both if the point defined by the two candidates is in one of the striped triangles in the figure. Hence the total probability of accepting a candidate in $[1-\delta,1]$ is at least $\delta^2$. 
%\end{proof}

\begin{figure}[t]
\begin{center}
\includegraphics[width=.3\textwidth]{./figs/delta}
\caption{The striped areas are the areas that if the point defined by the two candidates $(y_1,y_2)$ is in one of them then a candidate in the interval $[1-\delta/2,1]$ will join the group.  \label{fig-delta}  
}
\end{center}
\end{figure}


%
%In the following subsections we first show that the $p$-quantile will get to a location greater than $1/2$ and stay there. Next, we show that given that the $p$-quantile is above $1/2$ it will converge to $\tau_p$.
%\subsubsection{The $p$-quantile converges to a value greater than $1/2$}

%\begin{theorem} \label{thm-greater-than-half}
%Let $k_0$ be the initial size of the group. For $k_{min} > k_0$, with probability $1-  \sum_{k=k_{min}}^\infty e^{-\theta(k)}$, there exists $k_{1/2} >  k_{min}$ such that for every $k\geq k_{1/2}$, $q_p(S(k))>1/2$.
%\end{theorem}
\begin{theorem} \label{thm-veto-smooth}
Consider a group $S(k_0)$. There exists a time step $k_{1/2}$ such that with probability $1-o(1)$ for any $k'>k_{1/2}$ the admission rule is smooth.
\end{theorem}
\begin{proof}
Pick $\eta = \frac{p-1/2}{4}$. We will show that with high probability there exists $k_{1/2} > k_0$ such that $q_{p-\eta}(S(k_{1/2}))>1/2$ and for any $k'>k_{1/2}$, $q_{p}(S(k_{1/2}))>1/2$. This implies that the admission rule is smooth for any group of size greater than $k_{1/2}$.

%We will show that there exists $k_{1/2} > k_{min}$ such that $q_{p-\eta}(S(k_{1/2}))>1/2$ such that
% For $k_{min} > k_0$, with probability $1-\sum_{i=1}^{\infty} e^{-\Theta(\eta^3 (1+\eta)^{i-1} k_{min})}$, 

The proof follows a very similar structure to the proof of Theorem \ref{thm:conv:extreme}. We begin by showing that as we increase the group by $\eta k$ members at most $(p-2\eta) \cdot \eta k$ members will join the interval $[0, q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$.

\begin{claim} \label{clm:half-eps-k}
For a group $S(k)$ such that $q_{p-\eta}(S(k))<1/2$, consider adding $\eta k$ members to the group $S(k)$, with probability $(1-e^{-\Theta(\eta^3k)})$. The number of members that joined the interval $[0, q_{p-\eta}(S(k))+ \eta \cdot q_{p-\eta}(S(k))^2]$ in the $\eta k$ steps at most $(p-2\eta) \cdot \eta k$.
\end{claim}
\begin{proof}
Note that by definition we have that for every step $k'$ of the $\eta k$ steps, $q_{p}(S(k')) \geq q_{p-\eta}(S(k))$. We claim that this implies that the probability that the next accepted candidate is below $q_{p-\eta}(S(k)) + \eta \cdot q_{p-\eta}(S(k))^2$ is at most $p-3\eta$. To see why this is the case we first observe that with probability $ q_{p-\eta}(S(k))^2$ both candidates are below $q_{p-\eta}(S(k))$ and hence a candidate below $q_{p-\eta}(S(k))$ is accepted. Also note that with probability at most $2 \eta \cdot q_{p-\eta}(S(k))^2$ a member in the interval $[q_{p-\eta}(S(k)), q_{p-\eta}(S(k))+ \eta \cdot q_{p-\eta}(S(k))^2]$ joins the group, as this is an upper bound on the probability that a candidate in this interval shows up. Finally, as we only take into account steps in which a candidate was chosen we should divide the probabilities above by the probability of accepting a member. It it easy to see that the probability of accepting a member is minimized when $q_p(S(k')) = q_{p-\eta}(S(k))$ and hence the probability that the next accepted candidate is in the interval $[0, q_{p-\eta}(S(k))+ \eta \cdot q_{p-\eta}(S(k))^2]$ is at most 
\begin{align*}
\dfrac{q_{p-\eta}(S(k))^2 + 2 \eta \cdot q_{p-\eta}(S(k))^2}{2q_{p-\eta}(S(k))^2} = \dfrac{1}{2}+\eta = p-3\eta.
\end{align*}
By taking a Chernoff bound we get that with high probability the number of members accepted in the $\eta k$ steps in the interval $[0, q_{p-\eta}(S(k))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$ is at most $(p-2\eta) \cdot \eta k$. Denote by $X$ the number of candidates accepted in the interval $[0, q_{p-\eta}(S(k))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$, then
\begin{align*}
Pr[X\geq (1+\eta) \cdot (p-3\eta) \cdot \eta k] \leq e^{-\frac{\eta^2 (p-3\eta) \cdot \eta k}{3}} \leq e^{-\Theta(\eta^3k)}
\end{align*}
\end{proof}

Let $k_1 \geq\frac{1}{\eta^6}$ (the larger $k_1$ is, the higher the probability the theorem holds is) and for any $i>1$ let $k_{i+1} = (1+\eta) k_i$. Also let $j=\lceil \log_{1+\eta} \frac{1}{\eta} \rceil$. We show that with high probability: $q_{p-\eta}(S(k_{i+j})) > q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2$.

\begin{claim} \label{clm-half-decreasing}
For $i>1$, with probability $(1-\sum_{l=1}^{j-1} e^{-\Theta(\eta^3 (1+\eta)^lk_i)})$, either there exists $k_i<k'<k_{i+j}$ such that $q_{p-\eta}(S(k))>1/2$ or $q_{p-\eta}(S(k_{i+j})) > q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2$.
\end{claim}
\begin{proof}
To prove the claim we apply Claim \ref{clm:half-eps-k} $j$ times. First we observe that with high probability for every $i$, $q_{p-\eta}(S(k_{i+1})) \geq q_{p-\eta}(S(k_i))$. The reason for this is that by Claim \ref{clm:half-eps-k} we have that the number of members that joined in the $\eta k_i$ steps between $k_i$ and $k_{i+1}$ in the interval $[0, q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$ is at most $(p-2\eta) \cdot \eta k$. Since the interval $[0, q_{p-\eta}(S(k_i))]$ is included in this interval we have that at most $(p-2\eta) \cdot \eta k$ members were admitted to it. Hence, $q_{p-\eta}(S(k_{i+1})) \geq q_{p-\eta}(S(k_i))$.

Next, we consider all the members in the $k_{i+j}-k_i$ steps. The fact that $q_{p-\eta}(S(k_{i+1})) \geq q_{p-\eta}(S(k_i))$ implies that in the $k_{i+j}-k_i$ steps the number of candidates admitted to the interval $[0, q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$ is at most $(p-2\eta)(k_{i+j}-k_i)$. We observe that in the worst case for the group $S(k_i)$ the interval $[0, q_{p-\eta}(S(k_i))+ \eta \cdot q_{p-\eta}(S(k_i))^2]$ contained $k_i$ points. Thus, to prove the claim, we should show that $(p-2\eta)(k_{i+j}-k_i)+k_i < (p-\eta)k_{i+j}$. Observe that 
\begin{align*}
(p-2\eta)\cdot(k_{i+j}-k_i) + k_i &= (p-\eta)k_{i+j} -\eta k_{i+j} + (1-p+2\eta)k_i  \\
&< (p-\eta)k_{i+j} - k_{i} + (1-p+2\eta)k_i \\
&< (p-\eta)k_{i+j}.
\end{align*}
For the second transition we used the fact that $k_{i+j} = (1+\eta)^{\lceil \log_{1+\eta} \frac{1}{\eta} \rceil} k_i > \frac{1}{\eta} k_i$.

Thus by taking a union bound over the bad events we get that the claim holds with probability
at least 
\begin{align*}
1-\sum_{l=i}^{i+j-1} e^{-\Theta(\eta^3 k_l)}. %= 1-\sum_{l=1}^{j-1} e^{-\Theta(\eta^3 (1+\eta)^lk_i)}
\end{align*}
\end{proof}

Lastly, we show that once we reached a step $k_i$ such that the $(p-\eta)$-quantile is above $1/2$, then with high probability the $p$-quantile of $S(k_{i+1})$ will also be above $1/2$.
\begin{claim} \label{clm:non-stays}
If $q_{p-\eta}(S(k_i)) > 1/2$, then with probability $(1-e^{-\Theta(\eta^3 k_i)}$, $q_{p-\eta}(S(k_{i+1})) > 1/2$
\end{claim}
\begin{proof}
Observe that since $q_{p} (S(k')) >1/2$ for all $k'$ of the $\eta k_i$ steps, the expected number of members accepted below $1/2$ in these $\eta k_i$ steps is at most $\frac{\eta k_i}{2}$. By taking a Chernoff bound, we have that with probability $1-e^{-\frac{\eta^3 k_i}{6}}$ the number of candidates accepted in $[0,1/2]$ is at most $(1/2+\eta)\eta k_i<(<p-\eta)k+i$:
\begin{align*}
Pr[X\geq (1+\eta) \cdot \frac{1}{2} \eta k_i] \leq e^{-\frac{\eta^2 \frac{1}{2} \eta k_i}{3}} = e^{-\frac{\eta^3 k_i}{6}}
\end{align*}
%The proof is completed by observing that $(1/2+\eta)<p-\eta = 1/2 + 3\eta$.
\end{proof}

The proof of Theorem is completed by observing that we can apply Claim \ref{clm-half-decreasing} till we reach $k_{1/2}$ such that $q_{p-\eta}(k_{1/2})>1/2$. Once we reached $k_{1/2}$ we repeatedly apply Claim \ref{clm:non-stays} to get that the $(p-\eta)$-quantile stays above $1/2$ with high probability. By taking a (loose) union bound over the bad events we have that the probability of this is at least $1-\sum_{i=1}^{\infty} e^{-\Theta(\eta^3 k_i)}$.
\end{proof}





%\subsubsection{The $p$-quantile Converges to $\tau_p$}
%We first provide the computation for the value of $\tau_p$. Recall that in the beginning of
%the section we argued that when the $p$-quantile is above $1/2$ the probability of accepting a candidate left of $q_p(S(k))$ is $f(q_p(S(k)))=\frac{q_p(S(k))^2}{1-2(1-q_p(S(k)))^2}$. Given this, the value of $\tau_p$ can be computed as follows:
%\begin{claim}
%The fixed point for the location of the $p$-quantile is:$\tau_p = \frac{2p + \sqrt{2p^2-p}}{1+2p}$.
%\end{claim}
%\begin{proof}
%As previously discussed since $\tau_p$ is a ``fixed point'' $(f(\tau_p)=p)$ then:
%\begin{align*}
%\frac{\tau_p^2}{1-2(1-\tau_p)^2} = p &\implies \tau_p^2 = p - 2p\tau_p^2 + 4p\tau_p -2p \\ &\implies (1+2p)\tau_p^2-4p\tau_p +p = 0.
%\end{align*}
%The solutions for this equation are
%\begin{align*}
%\tau_p = \frac{4p \pm \sqrt{16p^2 - 4p(1+2p)}}{2(1+2p)} = \frac{2p \pm \sqrt{2p^2-p}}{1+2p}.
%\end{align*}
%Recall that $f(q)$ is only defined for $q > 1/2$, thus we are only interested in points located above $1/2$. The only such point is $\tau_p = \frac{2p + \sqrt{2p^2-p}}{1+2p}$.
%\end{proof}
%
%We now show that the $p$-quantile converges to $\tau_p$. 




